The Potential of Subsampling and Inpainting for Fast Low-Dose Cryo FIB-SEM Imaging and Tomography

Traditional image acquisition for cryo focused ion-beam scanning electron microscopy tomography often sees thousands of images being captured over a period of many hours, with immense data sets being produced. When imaging beam sensitive materials, these images are often compromised by additional constraints related to beam damage and the devitrification of the material during imaging, which renders data acquisition both costly and unreliable. Subsampling and inpainting are proposed as solutions for both of these aspects, allowing fast and low-dose imaging to take place in the FIB-SEM without an appreciable low in image quality. In this work, experimental data is presented which validates subsampling and inpainting as a useful tool for convenient and reliable data acquisition in a FIB-SEM, with new methods of handling 3-dimensional data being employed in context of dictionary learning and inpainting algorithms using a newly developed microscope control software and data recovery algorithm.

==> fig_graveyard.tex <==
%% BIG ONE %%

\begin{figure*}
    \def\firstColWidth{0.08}
    \def\colWidth{0.22}
    \def\vertSpacing{0.25mm}

    \centering

    \begin{minipage}{\textwidth}
        \centering
        % row 0
        \begin{minipage}{\firstColWidth\textwidth}
            \centering
            Sampling Percentage
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \textbf{Inpainted Result} \\ (Frame 50)  
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \textbf{Integrated Result} \\ (100 Frames)
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \textbf{Integrated Result} \\ (100 Frames) CLAHE  
        \end{minipage}
    \end{minipage}

    \vspace{\vertSpacing}
    
    \begin{minipage}{\textwidth}
        \centering
 
        %row 1
        \begin{minipage}{\firstColWidth\textwidth}
            \begin{center}
                100\%
            \end{center}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/sample_frame_50_1.png}
        \end{minipage}        
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/integrated_1.png}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/CLAHE_1.png}
        \end{minipage}
       
    \end{minipage}

    \vspace{\vertSpacing}

    \begin{minipage}{\textwidth}
        \centering

        %row 2
        \begin{minipage}{\firstColWidth\textwidth}
            \begin{center}
                50\%
            \end{center}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/sample_frame_50_2.png}
        \end{minipage}        
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/integrated_0.5.png}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/CLAHE_0.5.png}
        \end{minipage}
       
    \end{minipage}

    \vspace{\vertSpacing}

    \begin{minipage}{\textwidth}
        \centering

        %row 3
        \begin{minipage}{\firstColWidth\textwidth}
            \begin{center}
                25\%
            \end{center}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/sample_frame_50_3.png}
        \end{minipage}        
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/integrated_0.25.png}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/CLAHE_0.25.png}
        \end{minipage}
       
    \end{minipage}

    \vspace{\vertSpacing}

    \begin{minipage}{\textwidth}
        \centering

        %row 4
        \begin{minipage}{\firstColWidth\textwidth}
            \begin{center}
                20\%
            \end{center}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/sample_frame_50_4.png}
        \end{minipage}        
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/integrated_0.20.png}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/CLAHE_0.20.png}
        \end{minipage}
       
    \end{minipage}

    \vspace{\vertSpacing}

    \begin{minipage}{\textwidth}
        \centering

        %row 5
        \begin{minipage}{\firstColWidth\textwidth}
            \begin{center}
                15\%
            \end{center}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/sample_frame_50_5.png}
        \end{minipage}        
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/integrated_0.15.png}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/CLAHE_0.15.png}
        \end{minipage}
       
    \end{minipage}

    \vspace{\vertSpacing}

    \begin{minipage}{\textwidth}
        \centering

        %row 6
        \begin{minipage}{\firstColWidth\textwidth}
            \begin{center}
                10\%
            \end{center}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/sample_frame_50_6.png}
        \end{minipage}        
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/integrated_0.10.png}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/CLAHE_0.10.png}
        \end{minipage}
       
    \end{minipage}

    \vspace{\vertSpacing}

    \begin{minipage}{\textwidth}
        \centering

        %row 7
        \begin{minipage}{\firstColWidth\textwidth}
            \begin{center}
                5\%
            \end{center}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/sample_frame_50_7.png}
        \end{minipage}        
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/integrated_0.05.png}
        \end{minipage}
        \begin{minipage}{\colWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/bigfig/CLAHE_0.05.png}
        \end{minipage}
       
    \end{minipage}

    \caption{Images of \textit{Euglena gracilis} at a variety of sampling percentages, and various processing steps. First, the data acquired from the microscope (examples in column one) is inpainted using BPFA (examples in column three). This set of reconstructions is then integrated through the data stack (column three) to form the final image. Histogram equalisation is applied to reduce contrast variations due to charging for data viewing purposes (column four).}
    \label{fig:main}
    
\end{figure*}


%% DEAD ONE %%

\begin{figure}
    \def\compH{0.2}
    \def\compHs{0.08}
    \def\compV{0.25mm}
    \centering

    \begin{minipage}{\textwidth}
        % row 0
        \begin{minipage}{\compHs\textwidth}
            \centering
            Sampling Percentage
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \centering
            \textbf{Sample Frame} \\ (Frame 50) 
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \centering
            \textbf{Integrated Result} \\ (100 Frames)  
        \end{minipage}
    \end{minipage}

    \vspace{\compV}


    %row 1
    \begin{minipage}{\textwidth}
        \begin{minipage}{\compHs\textwidth}
            \centering
            100\%
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/bigfig/raw_sample_frame_50_1.png}
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/raw_comparison/raw_integrated_stack_1.png}
        \end{minipage}
    \end{minipage}

    \vspace{\compV}
    
    %row 2
    \begin{minipage}{\textwidth}
        \begin{minipage}{\compHs\textwidth}
            \centering
            50\%
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/bigfig/raw_sample_frame_50_2.png}
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/raw_comparison/raw_integrated_stack_2.png}
        \end{minipage}
    \end{minipage}

    \vspace{\compV}
    
    %row 3
    \begin{minipage}{\textwidth}
        \begin{minipage}{\compHs\textwidth}
            \centering
            25\%
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/bigfig/raw_sample_frame_50_3.png}
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/raw_comparison/raw_integrated_stack_3.png}
        \end{minipage}
    \end{minipage}

    \vspace{\compV}
    
    %row 4
    \begin{minipage}{\textwidth}
        \begin{minipage}{\compHs\textwidth}
            \centering
            20\%
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/bigfig/raw_sample_frame_50_4.png}
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/raw_comparison/raw_integrated_stack_4.png}
        \end{minipage}
    \end{minipage}

    \vspace{\compV}
    
    %row 5
    \begin{minipage}{\textwidth}
        \begin{minipage}{\compHs\textwidth}
            \centering
            15\%
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/bigfig/raw_sample_frame_50_5.png}
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/raw_comparison/raw_integrated_stack_5.png}
        \end{minipage}
    \end{minipage}

    \vspace{\compV}
    
    %row 6
    \begin{minipage}{\textwidth}
        \begin{minipage}{\compHs\textwidth}
            \centering
            10\%
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/bigfig/raw_sample_frame_50_6.png}
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/raw_comparison/raw_integrated_stack_6.png}
        \end{minipage}
    \end{minipage}

    \vspace{\compV}
    
    %row 7
    \begin{minipage}{\textwidth}
        \begin{minipage}{\compHs\textwidth}
            \centering
            5\%
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/bigfig/raw_sample_frame_50_7.png}
        \end{minipage}
        \begin{minipage}{\compH\textwidth}
            \includegraphics[width=\textwidth]{Figures/raw_comparison/raw_integrated_stack_7.png}
        \end{minipage}
    \end{minipage}



    
    \caption{Left column shows individual images of \textit{Euglena gracilis} at various sampling percentages. Right column shows the integrated stack of all frames (100) for each sampling percentage. Without inpainting, this integrated data still retains significant information when operating at relatively low sampling percentages. }
    \label{fig:enter-label}
\end{figure}

%% ANTI JEOL GANG %%

\begin{figure*}
    \def\demoFigWidth{0.499}
    \centering
    \begin{minipage}{\textwidth}
        \begin{minipage}{\demoFigWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/jeol130ns-1000int.png}
        \end{minipage}
        \begin{minipage}{\demoFigWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/senseAI1000ns-100int.png}        
        \end{minipage}
    \end{minipage}
    
    \vspace{0.8mm}
    
    \begin{minipage}{\textwidth}
        \begin{minipage}{\demoFigWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/jeol130ns-1000int-hist.png}
        \end{minipage}
        \begin{minipage}{\demoFigWidth\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/senseAI1000ns-100int-hist.png}       
        \end{minipage}
    \end{minipage}

    \caption{(Top, Left) SEM secondary electron integrated image formed by JEOL software; 130 \textit{ns} dwell time, 1000 frames. (Top, Right) SEM secondary electron integrated image formed by SenseAI software; 1 \textit{us} dwell time, 100 frames. Average electron probe exposure per pixel is 130us and 100us respectively. (Bottom) The images from the top row with post-integration histogram equalisation applied to reduce charging artefacts and are provided here for visualisation purposes. Images formed using SenseAI exhibit enhanced contrast and resolution at electron doses comparable to the JEOL software acquisition. Flyback distortions are present in the SenseAI-produced images as no flyback compensation is performed, as with the JEOL images.}
    \label{fig:demonstration}
\end{figure*}
